F-IVM: Learning over Fast-Evolving Relational Data

F-IVM is a system for real-time analytics such as machine learning applications over training datasets defined by queries over fast-evolving relational databases. We will demonstrate F-IVM for three such applications: model selection, Chow-Liu trees, and ridge linear regression.

==> scenario.tex <==
\nop{
\section{Demonstration Scenarios}

% \noindent
% \textbf{Applications.  }
% - Gradient Computation
% - Matrix Chain Multiplication




which are used to forecast user demand and sales.

The Retailer database has 87M tuples and 1.5GB size on disk. The natural join of 5 relations with 43 attributes in total has 87M tuples and 18GB size on disk.
  
It is implemented on top of the DBToaster backend~\cite{DBT:VLDBJ:2014}, which provides state-of-the-art code optimization and compilation for incremental maintenance of relational queries over databases. F-IVM replaces DBToaster's frontend with a new frontend that supports efficient maintenance strategies for batches of aggregates instead of individual aggregates. Furthermore,  F-IVM provides novel rings to capture expressive dynamic computation necessary for the maintenance of common relational learning applications. Using rings, both inserts and deletes are treated alike by F-IVM. Also, by changing the meaning of the sum and product ring operators as well as of the ring support, the same symbolic computation expressed using sums and products over elements from the ring support may capture the behavior of different applications.


We demonstrate the maintenance of the cofactor matrices 
for learning regression models over natural joins. 
We compute the cofactor matrices over all attributes, which suffices to learn linear regression models over any label and set of features that is a subset of the attributes.

We demonstrate F-IVM on three datasets: 
(1) \textit{Retailer} is a real-world dataset used to forecast user demands and sales. 
% A scenario is to predict how many inventory units a store should keep in order to satisfy the predicted demand.
It has a snowflake schema with one fact table \texttt{Inventory} with 87M tuples.
The natural join of five relations with 43 attributes in total has 87M tuples and 18GB size on disk.
(2) \textit{Housing} is a public synthetic dataset modeling a house price market~\cite{Nikolic:SIGMOD:18}. 
It consists of six relations, arranged into a star schema and with 1.4M tuples in total (scale factor 20). 
The natural join of all relations is on the common attribute (\texttt{postcode}) and has 27 attributes.
(3) \textit{Twitter} represents the connection relationships among users who were active on Twitter during the discovery of Higgs boson~\cite{snapnets}. 
We split the first 3M records from the dataset into three equally-sized relations, 
$R(A, B)$, $S(B, C)$, and $T(C, A)$, and consider the triangle query over them. 

% how to create the bulk of updates
We run the systems over data streams synthesized from the above datasets by interleaving insertions to the all relations in a round-robin fashion. 
We group insertions into batches of different sizes (varying from 100 to 100,000) and place no restriction on the order of records in input relations. 

}
